Prompt Waywardness: The Curious Case of Discretized Interpretation of Continuous Prompts

Fine-tuning continuous prompts for target tasks has recently emerged as a compact alternative to full model fine-tuning. Motivated by these promising results, we investigate the feasibility of extracting a discrete (textual) interpretation of continuous prompts that is faithful to the problem they solve. In practice, we observe a "wayward" behavior between the task solved by continuous prompts and their nearest neighbor discrete projections: We can find continuous prompts that solve a task while being projected to an arbitrary text (e.g., definition of a different or even a contradictory task), while being within a very small (2%) margin of the best continuous prompt of the same size for the task. We provide intuitions behind this odd and surprising behavior, as well as extensive empirical analyses quantifying the effect of various parameters. For instance, for larger model sizes we observe higher waywardness, i.e, we can find prompts that more closely map to any arbitrary text with a smaller drop in accuracy. These findings have important implications relating to the difficulty of faithfully interpreting continuous prompts and their generalization across models and tasks, providing guidance for future progress in prompting language models.

==> old_text.tex <==
% Fine-tuning continuous prompts are shown to enjoy competitive performance while being compact, making them  a promising alternative to architecture fine-tuning. 
% while necessitating a much smaller set of parameters.  
% the recent successes of fine-tuning continuous prompts for solving tasks, 
% describes the problem it solves.  
% there any correspondences between the discrete interpretation of continuous prompts and the tasks they solve. 
% Such correspondence could provide some level of interpretability into the behavior of continuous prompts.
% \kyle{a certain wayward behavior with respect to the resulting prompts, namely that there is often little connection}\kyle{**This sentence sounds a bit funny in its current form**}
% \lianhui{I feel like “their  nearest  neighbor  discrete  (textual) projections” may be a bit too specific and confusing ——readers may wonder why  “nearest neighbor”.  I guess we may just use more abstract expression, e.g “their discrete  (textual) projections” or  “their discrete  (textual) interpretations”.}
% \daniel{that's how it was phrased previously; the comment was that "projection" or "discrete projections" is not quite well-defined.} \lianhui{sure, makes sense to me}
% for \emph{any} random discrete statement, we empirically show the existence of continuous prompts that are mapped to this given text while providing a near-perfect solution to the target task. 
% we observe that the effect of waywardnness becomes worse (continuous prompts that are mapped to an arbitrary text while compromising little in task accuracy)

% \daniel{needs to be re-done after the experiments are there.}
% \daniel{you start with a story about a desired task that one can do: 
% like, differentiable prompt optimization 
% }

    \begin{tabular}{llccc @{\hspace{0.8em}} c}
    \toprule
        \multirow{2}{*}{Data} & $p_d$ & Acc (\%)  & \multirow{2}{*}{$\hat{\Delta}$ (\%)} & Prompt  \\
        & Source & $p_c^* \rightarrow \tilde{p}_c$ & & F1 (\%) \\
    \midrule
        \multirow{3}{*}{SST-2} 	& NI & 92.4 $\rightarrow$ 91.8  & 0.7   & 99.0\\
        & PILE & 92.5 $\rightarrow$ 92.0    & 0.5   & 97.1\\
        & Avg & 92.4 $\rightarrow$ 91.9	& 0.6	& 98.1 \\
    \cmidrule(lr){1-5}
        \multirow{3}{*}{SST-5} & NI	& 50.2 $\rightarrow$ 48.5   & 3.3   & 95.9\\
        & PILE & 50.5 $\rightarrow$ 50.2    & 0.7   & 92.4\\
        & Avg & 50.3 $\rightarrow$ 49.3 	& 2.0	& 94.2	\\
    \cmidrule(lr){1-5}
        \multirow{3}{*}{AGNews} & NI	& 88.0 $\rightarrow$ 86.6   & 1.6   &97.4\\
        & PILE & 88.1 $\rightarrow$ 88.2    & -0.1  & 97.5\\
        & Avg & 88.1 $\rightarrow$ 87.3	& 0.8	& 97.4 \\
    \cmidrule(lr){1-5}
        \multirow{3}{*}{Subj} & NI	& 91.3 $\rightarrow$ 89.5   & 2.0   & 97.3\\
        & PILE & 89.6 $\rightarrow$ 88.8    & 0.9   & 94.4\\
        & Avg & 90.5 $\rightarrow$ 89.2	& 1.5	& 95.9 \\
    \cmidrule(lr){1-5}
        \multirow{3}{*}{TREC} & NI	& 87.5 $\rightarrow$ 84.7   & 3.3   & 86.5\\
        & PILE & 88.5 $\rightarrow$ 87.5    & 1.2   & 85.6\\
        & Avg & 88.0 $\rightarrow$ 86.0	& 2.3	& 86.1 \\
    \bottomrule 
    \end{tabular}


\begin{conjecture}
    \label{conjecture:1}
    {\bf (controlled generation): }
    For \underline{any} target discrete prompt $p_d$ with length $L$ and a desired generation task  $y$, there always exists a continuous prompt $\tilde{p}_c \in \reals^{d\times L}$ such that: 
    (1) $\tilde{p}_c$ is a good solution for the target task compared to the optimal prompt $p^*_c$ (Eq.\ref{eq:optimal:1}), i.e.,  $|\ell(\tilde{p}_c; y)- \ell(p^*_c; y)| < \varepsilon$ for a small $\varepsilon$, yet 
    % it is a strong-enough minimizer of the
    (2) it is projected to the given (potentially, irrelevant) discrete prompt $p_d$: $d$-proj$(\tilde{p}_c) \approx p_d$.
\end{conjecture}


\begin{figure*}
    \centering
    \includegraphics[scale=0.78,trim=0.45cm 0.8cm 0.1cm 0.4cm]{figure/summary-fig-1.pdf}
    \caption{
    (a) \emph{Any} given discrete prompts has \emph{infinite} corresponding continuous prompts each solving a different task. (b) A key implication of \shortname{} is that immature attempts to interpret continuous prompts can result in vulnerabilities against malicious attacks concealed under the disguise of benign discrete representation. 
    For example, a  continuous prompt touted as a fair resume selection model based on its its discrete interpretation might be carrying egregious biases.   
    (c) While discrete prompts trigger similar behavior across models, the current continuous prompt technology is unlikely show meaningful zero-shot transfer because they are not tied the semantics carried by the discrete space. 
    }
    \label{fig:page2}
\end{figure*}
 
 
 % One might wonder why \shortname{} is happening. 
While it is difficult to provide a formal proof of this behavior, we provide intuition (\S\ref{subsec:intuiton}) to make sense of it. 
Intuitively, this phenomenon is enabled by the combination of two factors (Fig.\ref{fig:page2}-a): 
%  \emph{Any} given discrete prompts has \emph{infinite} corresponding continuous prompts each solving a different task.
(1) \emph{any} projection of continuous prompts into discrete space is many-to-one. 
% meaning that there are regions with infinite continuous prompts that are projected to the same discrete form (Fig.). 
(2) The expressivity of deep models empower continuous prompts to solve a variety of tasks, no matter how close they are to each other. 
\sameer{this seems too much for the intro.. I think stick to your contributions: ``we provide theoretical intuition behind why this might happen.'' or something.}\tushar{+1}

 
 
     \begin{tabular}{llrr @{\hspace{0.8em}} r}
    \toprule
        Dataset & $\gamma$ & Acc & $\Delta$ (\%) & Prompt F1 \\
    \midrule
        \multirow{3}{*}{\makecell[l]{SST-2 \\ (92.4)}}
        & 0.01	    & 91.9	& 0.6	& \textbf{\underline{98.1}} \\
        & 0.005     & 92.0	& 0.4	& 94.0 \\
        & 0.003	    & 92.1	& \textbf{\underline{0.3}}	& 87.7 \\
    \midrule
        \multirow{3}{*}{\makecell[l]{SST-5 \\ (50.3)}}
        & 0.01	    & 49.3	& 2.0	& \textbf{\underline{94.2}}	\\
        & 0.005	    & 49.6	& 1.5	& 81.9 \\
        & 0.003	    & 49.6	& \textbf{\underline{1.4}}	& 71.2	\\
    \midrule
        \multirow{3}{*}{\makecell[l]{AGNews \\ (88.1)}}
        & 0.01	    & 87.3	& \textbf{\underline{0.8}}	& \textbf{\underline{97.4}} \\
        & 0.005	    & 87.1	& 1.0	& 92.2 \\
        & 0.003	    & 87.2	& 9.3	& 83.0 \\
    \midrule
        \multirow{3}{*}{\makecell[l]{Subj \\ (90.5)}}
        & 0.01	    & 89.2	& 1.5	& \textbf{\underline{95.9}} \\
        & 0.005	    & 89.2	& 1.4	& 90.7 \\
        & 0.003	    & 89.9	& \textbf{\underline{0.7}}	& 86.5  \\
    \midrule
        \multirow{3}{*}{\makecell[l]{TREC \\ (88.0)}}
        & 0.01	    & 86.0	& 2.3	& \textbf{\underline{86.1}} \\
        & 0.005	    & 87.2	& \textbf{\underline{0.9}}	& 66.2 \\
        & 0.003	    & 87.2	& 1.0	& 52.5 \\
        \bottomrule 
    \end{tabular}
    
    
\begin{figure*}[!th]
    \centering
    \includegraphics[scale=0.38]{figure/effect_of_prompt_length_and_size_1.pdf}
    \includegraphics[scale=0.38]{figure/effect_of_prompt_length_and_size.pdf} 
    %\rule{6cm}{1cm}
    \caption{
    \daniel{brought back the previous version of the figure. tops how shows absolute accuracy; bottom shows their gap. I think to show the whole picture, we may want to include both figures. }
    \textbf{(Left and middle)}
    The effect of the length of the prompt ($L$) on SST-2 and AGNews.
    %{\em Relative Accuracy Drop} (green) is calculated against unconstrained accuracy, and is averaged over 32 discrete prompts from Natural Instructions and 3 random seeds ($\gamma=0.01$ used).
    {\em Accuracy} (green) and {\em unconstrained accuracy} (blue) are averaged over 32 discrete target prompts from Natural Instructions and 3 random seeds ($\gamma=0.01$ used).
    The corresponding prompt F1 is reported as a orange line.
    \textbf{The relative accuracy drop is marginal when $L$ is not too small (e.g. 7 or larger).}
    \textbf{(Right)}
    The effect of the size of the model---small, medium, large, and XL---on SST-2.
    {\em Accuracy} (green) and {\em unconstrained accuracy} (blue) are averaged over 30 discrete target prompts from The PILE and 3 random seeds.
    We vary $\gamma=\{0.01, 0.005, 0.003\}$ and choose the one for which prompt F1 is larger than 0.98.
    \textbf{The relative accuracy drop decreases as models become larger.}\tushar{Reaffirm that pc* also uses the same length}\daniel{confirmed: they are used in the same length.}
    }
    \label{fig:ablation_prompt_len_size}
\end{figure*}

\begin{comment}
Nearest-neighbor projections are arguably natural, computationally efficient, and useful in practice. Although we have considered them in the Euclidean space so far, they can be defined for an \emph{arbitrary} distance metric\footnote{\url{https://en.wikipedia.org/wiki/Metric_(mathematics)}} $m$ on $\mathbb{R}^d$. As before, consider an embedding of a lexicon of size $V$ into $\mathbb{R}^d$ and the corresponding one-hot vectors in $\{0,1\}^V$. We call $d\text{-proj}$ a \emph{nearest-neighbor projection operator w.r.t.\ $m$} if it maps each $x \in \mathbb{R}^d$  to the one-hot vector in $\{0,1\}^V$ that corresponds to the lexicon item whose embedding is closest to $x$ under metric $m$ (breaking ties arbitrarily).

\begin{proposition}
\label{prop:nnbr-projections}
    Every nearest-neighbor projection operator, under any metric, maps infinitely many elements of $\mathbb{R}^d$, forming one or more continuous subspaces, to every one-hot vector in $\{0,1\}^V$.
\end{proposition}

A proof is included in the Appendix. In effect, the projection operators induce a clustering of the space of continuous prompts $\mathbb{R}^{d\times L}$ into regions that have the same discrete projection (Fig.\ref{fig:clustering}). 

\begin{figure}[tb]
    \centering
    % \includegraphics[trim=0cm 0.5cm 0cm 0.5cm, scale=0.7]{figure/vorooni-1.pdf}
    % \includegraphics[trim=0.5cm 0.9cm 0cm 0.9cm, scale=0.8]{figure/vorooni-2.pdf}
    \includegraphics[trim=0.65cm 0.9cm 0cm 0.5cm, scale=0.9]{figure/vorooni-3.pdf}
    \caption{The projection discrete space (Eq.\ref{eq:dproj}) induces a clustering (a Voronoi diagram) of the continuous space. Each cluster has infinitely many points that get mapped to the same discrete token. 
    % \daniel{be explicit that this is for a fixed position.}
    }
    \label{fig:clustering}
\end{figure}

The infinite-to-one mapping aspect is not limited to
% a particular choice of projection operator (Eq.\ref{eq:dproj}) or even to 
the class of nearest-neighbor projection operators. It is rather an inherent property of the interaction between continuous and discrete spaces, and holds for a broader family consisting of all but a negligible portion of possible projection operators:
% The following result states that the aforementioned result hold for a much broader family of projection functions. 
% \daniel{hanna was suggesting maybe we should change this to an "axiom" or just say it in the text in the passing, if we feel that our proof is not rigorous enough.}
% \begin{lemma}
% \label{lemma:1}
% For any projection operator $d\text{-proj}$ that maps $\mathbb{R}^d$ into one-hot vectors in $\{0, 1\}^V$, there are infinite continuous prompts that can be projected onto a fixed discrete target prompt. 
% \end{lemma}
% \begin{proof}
% Any $d$-projection operator partitions $\mathbb{R}^d$ (an infinite space) into $V$ partitions. 
% Therefore, based on the pigeonhole principle there always exists at least a portioned region with infinite points. \tushar{Should we say something about degenerate projections where infinite points are mapped to a special vocabulary item and the remaining V-1 items only have a single point? We seem to be claiming that every discrete target prompt will have infinite continuous prompts. But the pigeonhole principle only proves that at least one discrete prompt will have infinite continuous prompts.}
% \end{proof}

\begin{proposition}
\label{prop:infinite-to-one}
    Let $\mathbb{D}$ denote the space of all projection operators that map $\mathbb{R}^d$ to one-hot vectors in $\{0,1\}^V$. Let $d\text{-proj}$ be a random projection drawn uniformly from $\mathbb{D}$. Then, with probability 1, $d\text{-proj}$ maps infinite elements of $\mathbb{R}^d$ to every one-hot vector in $\{0,1\}^V$.
\end{proposition}


The above propositions indicate that there is a whole region of continuous prompts that correspond to a fixed discrete representation (Fig.\ref{fig:clustering}). 
\end{comment}



\begin{comment}
% Another notable difference between different LMs is in terms of their directionality. 
% Even on models other than GPT$k$ that enjoy have different directionality (e.g., BERT~\cite{devlin2019bert} which is conditioned on inputs on both sides) we expect \shortname{} to hold for an appropriately-defined inputs. 
%  while for GPT$k$ models the prompt is typically the left context, other models such as BERT~\cite{devlin2019bert} are conditioned on the inputs on both sides. 
 Another notable difference between different LMs is the directionality i.e. left-to-right attention models such as GPT-2 vs bidirectional attention models such as BERT~\cite{devlin2019bert}. We expect \shortname{} to hold for continuous prompts for models with bi-directional attention~\cite{zhong2021factual} too 
for an appropriately-defined input prompts, 
% irrespective of their attention patterns,
 since we would still have infinitely many continuous prompts mapping to the same discrete prompt.
 %\tushar{Can we add a cite for prompt-tuning for BERT-style model?} 
 %\daniel{not that I know of.} \sewon{\citet{zhong2021factual}?} \daniel{Tushar, how do you think we should cite this work in this context?}
\sewon{If we want to cut some space, merging two paragraphs above seems to be possible, since both are discussing about how our work can be easily extended to other LM models (including bidirectional ones instead of unidirectional) and other projection operators.}

\yejin{I am pretty uncomfortable about the confident speculations made by the previous paragraph without solid empirical backups...}\ashish{I would just drop the previous paragraph. And then also drop the title of the paragraph "Extent of the findings".  Just finish with a 3 paragraph section.}
\end{comment}


